A study of the local dynamics of modified Patankar DeC and higher order modified Patankar RK methods

Patankar schemes have attracted increasing interest in recent years because they preserve the positivity of the analytical solution of a production-destruction system (PDS) irrespective of the chosen time step size. Although they are now of great interest, for a long time it was not clear what stability properties such schemes have. Recently a new stability approach based on Lyapunov stability with an extension of the center manifold theorem has been proposed to study the stability properties of positivity-preserving time integrators. In this work, we study the stability properties of the classical modified Patankar--Runge--Kutta schemes (MPRK) and the modified Patankar Deferred Correction (MPDeC) approaches. We prove that most of the considered MPRK schemes are stable for any time step size and compute the stability function of MPDeC. We investigate its properties numerically revealing that also most MPDeC are stable irrespective of the chosen time step size. Finally, we verify our theoretical results with numerical simulations.

==> conclusion.tex <==
\section{Conclusion}\label{se_conclusion}

In this paper, we have investigated the stability conditions for several modified Patankar schemes. We were able to demonstrate that the MPRK(3,2) scheme proposed in \cite{torlo2021issues} and the MPRK43($\gamma$) schemes from \cite{kopecz2018unconditionally} are stable considering  general positive linear $N\times N$ systems. Further, we  provided the stability functions for the MPRK43($\alpha, \beta)$ schemes and derived several conditions \eqref{eq:assumption.prop.MPRK43(alpha,beta)} on the parameters to obtain a stable scheme. 
For a fixed method, the conditions \eqref{eq:assumption.prop.MPRK43(alpha,beta)} can easily be checked whereas through a numerical study we have concluded that these conditions should be as well fulfilled for the general  parameter selection. However, a formal proof is still missing. This remaining investigation will also be part of future research.  Besides this analysis, we have also considered the arbitrary high-order MPDeC schemes when applied to the $2\times 2$ system \eqref{PDS_test}. We were able to compute the stability function for several MPDeC schemes and investigated the schemes numerically. We have seen that using Gauss-Lobatto points, we always obtain a stable scheme whereas for equispaced points stability issues have been recognized for higher-order methods and large $\Delta t$. This fact is not surprising since already DeC methods show stability issues  if equispaced points are used and also the investigation  in \cite{torlo2021issues} confirms those problems. We have seen that the $\Delta t$ bound can be estimated from stability functions and eigenvalues.

In the future, we plan to continue our investigation in several directions. First, we consider the MPDeC schemes for more general systems numerically or even analytically. Then, we want to merge the stability investigation with the study in \cite{torlo2021issues}. Finally, also non-conservative Patankar systems as the ones proposed in \cite{chertock2015steady} will be studied next. 



